Simultaneous Object Reconstruction and Grasp Prediction using a Camera-centric Object Shell Representation

Being able to grasp objects is a fundamental component of most robotic manipulation systems. In this paper, we present a new approach to simultaneously reconstruct a mesh and a dense grasp quality map of an object from a depth image. At the core of our approach is a novel camera-centric object representation called the "object shell" which is composed of an observed "entry image" and a predicted "exit image". We present an image-to-image residual ConvNet architecture in which the object shell and a grasp-quality map are predicted as separate output channels. The main advantage of the shell representation and the corresponding neural network architecture, ShellGrasp-Net, is that the input-output pixel correspondences in the shell representation are explicitly represented in the architecture. We show that this coupling yields superior generalization capabilities for object reconstruction and accurate grasp quality estimation implicitly considering the object geometry. Our approach yields an efficient dense grasp quality map and an object geometry estimate in a single forward pass. Both of these outputs can be used in a wide range of robotic manipulation applications. With rigorous experimental validation, both in simulation and on a real setup, we show that our shell-based method can be used to generate precise grasps and the associated grasp quality with over 90% accuracy. Diverse grasps computed on shell reconstructions allow the robot to select and execute grasps in cluttered scenes with more than 93% success rate.

==> grasping.tex <==
\section{Grasping on Object Reconstruction}
\label{sec:grasping}
%
\begin{figure}
\centering
\includegraphics[scale=0.225]{figures/robot_expsetup.png}
\caption{Our experimental setup with the set of test objects.}
\label{fig:robot_setup}
\vspace{-5mm}
\end{figure} 
%
In this section, we explore the application of object shell representation for facilitating parallel-jaw grasp planning. 
% First we demonstrate that grasps can be sampled and evaluated for grasp feasibility and quality using the reconstructed mesh. Next we further show that by adding more channels to the decoder of the reconstruction network we can predict per pixel grasp feasibility and grasp quality on the input depth image avoiding the need for sampling or exploration for good feasible grasps. 
%Using both the geometry from the shell reconstruction and localization of the high quality grasp feasible regions from the  grasp feasibility and quality maps, we get set of dense high quality feasible grasps.
A parallel-jaw grasp can be defined by a grasp pose - the position and orientation of the gripper, and grasp width - the distance between the fingers.

% \subsection{Grasp Predictions using reconstructed mesh}
% \label{sec:grasp_sampling}
% In this section, we use the reconstructed mesh for sampling dense dense grasp proposals  and evaluating their grasp feasibility, grasp width, and grasp quality. 

% The reconstructed object shell mesh or pointcloud can be directly used with a standard grasp planning tools such as GraspIt~\cite{miller04graspit} or input to learning-based methods such as GPD, Contact-GraspNet~\cite{tenPas17gpd, sundermeyer2021contact} to generate grasps. 
% In this section, first we describe a basic scheme for sampling dense grasps proposals and characterizing them for their feasibility and quality using object shell reconstruction. 
% Then, we propose a joint network for object shell reconstruction and grasp prediction which outputs object shell as well as per pixel grasp feasibility and quality directly from the input depth image of the object.

\myparagraph{Grasp Feasibility and Grasp Width Computation}:
\label{sec:grasp_feas}
As shown in \figref{fig:shell_use}-(d), we sample grasps on the visible pointcloud of the object and use the object reconstruction to evaluate grasp feasibility. We assign a grasp pose such that the axis joining the fingers (finger axis) is along the point normal and one of the fingers is over the visible pointcloud with the full ($85$~mm) gripper opening.
A grasp is geometrically feasible if the local object geometry is within the gripper opening and does not collide with the gripper. 
%We further impose a constraint that the normals at the set threshold number of points on the object reconstruction inside the gripper envelope need to be along the finger axis. 
For a fixed grasp position, the grasp orientation is changed about the finger axis (to eight discrete angles covering 360$^{\circ}$). For all the feasible grasps, we compute the required grasp width from the bounds of the reconstruction inside the gripper envelope along the finger axis.
%
In \secref{sec:geom_grasp_eval}, we show that evaluating the accuracy of the grasp width prediction serves as a good metric to understand how object reconstruction accuracy affects grasp planning. From the application point of view, precise grasp width estimation is useful for grasping in clutter to avoid collision with the other objects.

\myparagraph{Grasp Quality}:
\label{sec:grasp_q}
A commonly accepted grasp quality metric is a measure of the external wrench the grasp can resist~\cite{FerrariCanny92}. 
From the mechanics of a parallel-jaw grasp~\cite{Roa14graspq} (details in \appref{app:grasp_mech}~\cite{shellgrasping2021}), the grasp quality is inversely proportional to the Euclidean distance of the grasp position from the center of geometry of the object which can be obtained from the object reconstruction.
We generate a \textit{Grasp Quality Map} (\figref{fig:shell_use}e) where every feasible grasp is assigned a relative quality score between 0 and 1 based on its Euclidean distance from the center of the object reconstruction.

% In \secref{sec:real_grasp_eval}, with experiments in Mujoco simulator as well as on a real robot, we show that under external disturbance, the grasps of higher estimated quality succeed more than those with lower quality.


